A Tale of Two Features: Stable Diffusion Complements DINO for Zero-Shot Semantic Correspondence

Text-to-image diffusion models have made significant advances in generating and editing high-quality images. As a result, numerous approaches have explored the ability of diffusion model features to understand and process single images for downstream tasks, e.g., classification, semantic segmentation, and stylization. However, significantly less is known about what these features reveal across multiple, different images and objects. In this work, we exploit Stable Diffusion (SD) features for semantic and dense correspondence and discover that with simple post-processing, SD features can perform quantitatively similar to SOTA representations. Interestingly, the qualitative analysis reveals that SD features have very different properties compared to existing representation learning features, such as the recently released DINOv2: while DINOv2 provides sparse but accurate matches, SD features provide high-quality spatial information but sometimes inaccurate semantic matches. We demonstrate that a simple fusion of these two features works surprisingly well, and a zero-shot evaluation using nearest neighbors on these fused features provides a significant performance gain over state-of-the-art methods on benchmark datasets, e.g., SPair-71k, PF-Pascal, and TSS. We also show that these correspondences can enable interesting applications such as instance swapping in two images.

==> tables/dino_analysis.tex <==
\begin{table}[ht]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.05}
\caption{\textbf{Performance comparison of DINOv2 variants.} Each variant attempts to enhance the DINOv2 features by addressing its limitations. Filter-ViT-B/14 employs a bilateral filter for smoothness, while Ensemble-ViT-B/14 combines early and last layers to capture more spatial information. We also include the result of our method, Fused-ViT-B/14, for reference.
}
\label{tab:dino_analysis}
\vspace{0.5em}
\begin{tabular}{@{}l @{\hskip 2.2em} cccccccccc}
\toprule
&\multicolumn{3}{c}{SPair-71k}&\multicolumn{3}{c}{PF-Pascal}&\multicolumn{4}{c}{TSS, PCK@0.05}\\
\cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-11}
  {Method}  & 0.01 & 0.05 & 0.10 & 0.05 & 0.10 & 0.15 & FG3DCar &JODS& Pascal & Avg.\\  
\midrule

DINOv2-ViT-B/14& 5.8 & 40.0 & 55.4&61.1&77.3&83.3&82.8&{{73.9}}&53.9&72.0\\
Filter-ViT-B/14& 4.7 & 37.4 & 55.3&61.6&79.0&84.6&86.4&{76.0}&{60.3}&76.2\\
Ensemble-ViT-B/14 & 6.4 & 40.7 & 56.1&62.6&79.7&86.1&84.7&{74.2}&59.7&74.8\\ \hline
Fuse-ViT-B/14 & 8.2 & 47.5 & 62.9&72.1&86.0&90.6&94.3&73.2&60.9&79.7\\
\bottomrule
\end{tabular}
\end{table}
